Green Application Placement in the Cloud-IoT Continuum

Green software engineering aims at reducing the environmental impact due to developing, deploying, and managing software systems. Meanwhile, Cloud-IoT paradigms can contribute to improving energy and carbon efficiency of application deployments by (i) reducing the amount of data and the distance they must travel across the network, (ii) by exploiting idle edge devices to support application deployment. In this article, we propose a declarative methodology and its Prolog prototype for determining placements of application services onto Cloud-IoT infrastructures so to optimise energy and carbon efficiency, also considering different infrastructure power sources and operational costs. The proposal is assessed over a motivating example.

==> src/background.tex <==
\section{Preliminaries}
\label{sec:background}

%In this section, we briefly present some concepts, notation and formulae that we will use next to define our model and to estimate energy consumption and carbon emissions. 

Greenhouse gases (GHG) are the direct cause of climate warming, by acting as a cover on the Earth's surface. While this is a totally natural phenomenon, human activities have dramatically accelerated it through the constant emission of high quantities of GHGs in the atmosphere \cite{microsoft}. The most common GHG is \textit{carbon dioxide} (\co ). For this reason, computations involving GHGs are usually performed by reducing all figures to \textit{carbon dioxide equivalent} (\coeq), and simply referring to GHGs as \textit{carbon}. 
%
Kelly et al. \cite{cotwo}, propose a methodology to associate an estimate of energy consumption and carbon emissions to a piece of computation running on a given server. The energy consumption $E_{c}$ of the a software service $c$ running on a server $s$ can be computed as

\begin{equation}\label{eq:energy}
E_{c} = E_{s} \cdot {PUE}_{s}
\end{equation}

\noindent
where $E_s$ is the current energy consumption of $s$ (in kWh) and ${PUE}_s$ is its \textit{power usage effectiveness}, i.e. the ratio between the energy that the server uses for actual computation and the energy needed for keeping the server working\footnote{For instance, a PUE of 1.5 indicates that for every 1kWh spent in computation, another 0.5kWh is needed for non-IT tasks that keep the server working. Typical values of the PUE range between $1.2$ and $1.9$.} (e.g. cooling, lighting, network). 
%
Note that, usually, $E_{s}=\phi(w)$ is a non-linear function of the current server workload $w$ \cite{microsoft}. Indeed, existing processors show a baseline energy consumption even when they are idle, which increases as the workload increases. For this reason, running a set of services on a lower number of servers, thus keeping the average workload per server higher, usually improves the overall \textit{energy efficiency} of the application deployment. 

Based on Eq. \ref{eq:energy}, it is then possible to estimate carbon emissions as:

\begin{equation}\label{eq:immissions}
I_{c} = \mu_{src} \cdot E_{c} 
\end{equation}

\noindent where $\mu_{src}$ are the average emissions of the power source that supplies the server onto which service $c$ is running, measured in \gcokw  . Pursuing the objectives of this paper, we extend Eq. \ref{eq:immissions} so to consider the case in which multiple energy  sources are used -- each with an associated probability $p_1, \dots, p_k$ such that $\sum_i p_i = 1$ -- producing $\mu_1, \dots, \mu_k$ emissions, respectively. 
%
Eq. \ref{eq:immissions} then becomes:

\begin{equation}\label{eq:immissions}
I_{c} = E_{c} \cdot \sum_i p_i \mu_i
\end{equation}

\noindent to account for energy mixes that are common in real deployments. Table \ref{tab:emissions} lists the emissions produced by different electricity sources.

\begin{table}[]
    \centering
\begin{tabular}{|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Power Source}} & \multicolumn{1}{c|}{\textbf{Emissions [$\text{kgCO}_2\text{/kWh}$]}} \\ \hline
\textit{gas}                                & 0.610                                                                \\ \hline
\textit{coal}                               & 1.100                                                                \\ \hline
\textit{on shore wind}                      & 0.0097                                                               \\ \hline
\textit{off shore wind}                     & 0.0165                                                               \\ \hline
\textit{solar}                              & 0.05                                                                 \\ \hline
\end{tabular}
\smallskip
    \caption{Emissions per power source \cite{cotwo}.}
    \label{tab:emissions}
\end{table}

Finally, following the methodology described in \cite{microsoft}, it is possible to estimate the carbon emissions needed to transmit 1MByte of information. Considering that 1MB of traffic requires on average $0.0023$ kWh to be transmitted through the Internet and that -- on average -- the \textit{global carbon intensity} of electricity is of 475 gCO2/kWh \cite{gci}, then the carbon emission $I_{t}$ for transmitting $m$ MB can be approximated as:

\begin{equation}\label{eq:immissions}
I_{t} = 0.0023 \cdot 475 \cdot m = 1.0925 \cdot m 
\end{equation}

Hence, when knowing the data rate in Mbit/s at which two services communicate, it is possible to (over)approximate the carbon footprint associated to such a communication by considering the MB exchanged within one hour, by simply knowing that 1 Mbit/s = 450 MB/h.

